Improved anomaly detection by training an autoencoder with skip connections on images corrupted with Stain-shaped noise

In industrial vision, the anomaly detection problem can be addressed with an autoencoder trained to map an arbitrary image, i.e. with or without any defect, to a clean image, i.e. without any defect. In this approach, anomaly detection relies conventionally on the reconstruction residual or, alternatively, on the reconstruction uncertainty. To improve the sharpness of the reconstruction, we consider an autoencoder architecture with skip connections. In the common scenario where only clean images are available for training, we propose to corrupt them with a synthetic noise model to prevent the convergence of the network towards the identity mapping, and introduce an original Stain noise model for that purpose. We show that this model favors the reconstruction of clean images from arbitrary real-world images, regardless of the actual defects appearance. In addition to demonstrating the relevance of our approach, our validation provides the first consistent assessment of reconstruction-based methods, by comparing their performance over the MVTec AD dataset, both for pixel- and image-wise anomaly detection.

==> Tables/RESULT_pixel-wise2.tex <==
\tabcolsep=0.075cm
\begin{table}[!h]
\begin{threeparttable}[b]
\caption{Pixel-wise detection AUC obtained with the residual- and uncertainty-based detection methods\tnote{a}. }
\label{table:summary_pixel-wise}
%\centering
\scriptsize
%\resizebox{\textwidth}{!}{

\newcommand\len{0.55}

\begin{tabularx}{8.9cm}{@{}llp{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}@{}} \toprule

%\multicolumn{2}{l}{Network} & \multicolumn{2}{c}{\textbf{AE}} & \multicolumn{3}{c}{\textbf{AESc}} & \textbf{AE\textsubscript{L2} \cite{Bergmann2019}} & \textbf{AE\textsubscript{L2} \cite{Dehaene2020}} & \textbf{AE\textsubscript{SSIM} \cite{Bergmann2019}} & \textbf{AE\textsubscript{SSIM} \cite{Dehaene2020}}  & \textbf{AnoGAN \cite{Bergmann2019}}\\

\multicolumn{2}{l}{Network} & \multicolumn{2}{c}{\textbf{AE}} & \multicolumn{3}{c}{\textbf{AESc}}  & \multicolumn{2}{c}{\textbf{AE\textsubscript{L2}}} & \multicolumn{2}{c}{\textbf{AE\textsubscript{SSIM}}} & \textbf{AnoGAN}\\

\arrayrulecolor{black!60}\cmidrule(lr){3-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
\multicolumn{2}{l}{Corruption} & None & Stain & None & \multicolumn{2}{c}{Stain} & \cite{Bergmann2019} & \cite{Dehaene2020} & \cite{Bergmann2019} & \cite{Dehaene2020} & \cite{Bergmann2019}\\

\arrayrulecolor{black!60}\cmidrule(lr){6-7}
&&&&& Res. & Un. &&&&&\\

\arrayrulecolor{black!60}\midrule\midrule

 \multirow{5}{*}{\rotatebox[origin=c]{90}{Textures}} & Carpet & 0.57 & 0.62 & 0.52 & 0.79 & \textbf{0.91} & 0.59 & 0.54 & \underline{0.87} & 0.55 & 0.54\\
& Grid & 0.81 & 0.82 & 0.57 & 0.89 & \underline{0.95} & 0.90 & \textbf{0.96} & 0.94 & \textbf{0.96} & 0.58 \\
& Leather & 0.79 & 0.82 & 0.71 & \textbf{0.95} & \underline{0.87} & 0.75 & 0.75 & 0.78 & 0.71 & 0.64\\ 
& Tile & 0.45 & 0.54 & 0.62 & \underline{0.74}  & \textbf{0.79} & 0.51 & 0.48 & 0.59 & 0.50 & 0.50 \\
& Wood & 0.64 & 0.71 & 0.65 & \textbf{0.84} & \textbf{0.84} & 0.73 & 0.63 & 0.73 & 0.64 & 0.62\\
\arrayrulecolor{black!60}\cmidrule(lr){2-12}
& Mean\tnote{b} & 0.65 & 0.70 & 0.61 & \underline{0.84} & \textbf{0.87} & 0.70 & 0.67 & 0.78 & 0.67 & 0.58\\
\arrayrulecolor{black!60}\midrule

 \multirow{10}{*}{\rotatebox[origin=c]{90}{Objects}} & Bottle &  0.85 & 0.88 & 0.47 & 0.84 & 0.88 & 0.86 & \underline{0.91} & \textbf{0.93} & \textbf{0.93} & 0.86 \\
& Cable & 0.62 & 0.83 & 0.72 & \underline{0.85} & 0.84 & \textbf{0.86} & 0.73 & 0.82 & 0.79 & 0.78 \\
& Capsule & 0.87 & 0.87 & 0.63 & 0.83 & \underline{0.93} & 0.88 & 0.79 & \textbf{0.94} & 0.77 & 0.84  \\
& Hazelnut & 0.92 & 0.93 & 0.79 & 0.88 & 0.89 & 0.95 & \textbf{0.98} & \underline{0.97} & \underline{0.97} & 0.87\\
& Metal Nut &  0.82 & 0.84 & 0.52 & 0.57 & 0.62 & 0.86 & \underline{0.88} & \textbf{0.89} & \underline{0.88} & 0.76\\
& Pill  & 0.81 & 0.81 & 0.64 & 0.74 & 0.85 & 0.85 & 0.89 & \textbf{0.91} & \underline{0.90} & 0.87\\
& Screw & 0.93 & 0.93 & 0.72 & 0.86 & 0.95 & \underline{0.96} & \textbf{0.98} & \underline{0.96} & \textbf{0.98} & 0.8  \\
& Toothbrush & 0.92 & \underline{0.93} & 0.73 & \underline{0.93} & \underline{0.93} & \underline{0.93} & \textbf{0.97} & 0.92 & \textbf{0.97} & 0.90\\
& Transistor & 0.79 & 0.82 & 0.56 & 0.80 & 0.78 & \underline{0.86} & \textbf{0.90} & \textbf{0.90} & \textbf{0.90}  & 0.8 \\
& Zipper & 0.73 & 0.75 & 0.60 & 0.78 & \textbf{0.90} & 0.77 & 0.68 & \underline{0.88} & 0.83 & 0.78\\
\arrayrulecolor{black!60}\cmidrule(lr){2-12}
& Mean\tnote{c} & 0.83 & 0.86 & 0.64 & 0.81 & 0.86 & 0.88 & 0.87 & \textbf{0.91} & \underline{0.89} & 0.82\\
\arrayrulecolor{black!60}\midrule

& Global mean\tnote{d} & 0.77 & 0.81 & 0.63 & \underline{0.82} & \textbf{0.86} & \underline{0.82} & 0.80 & \textbf{0.86} & \underline{0.82} & 0.74 \\
\arrayrulecolor{black}\bottomrule

\end{tabularx}
\begin{tablenotes}
\item [a]For each row, the best performing approach is highlighted in boldface and the second best is underlined.
\item [b] Mean AUC obtained over the classes of images belonging to the texture categories.
\item [c] Mean AUC obtained over the classes of images belonging to the object categories.
\item [d] Mean AUC obtained over the entire dataset.
\end{tablenotes}
\end{threeparttable}

\vspace*{-0.2cm}
%}
\end{table}

==> Tables/RESULT_pixel-wise3.tex <==
\tabcolsep=0.075cm
\begin{table}[!h]
\begin{threeparttable}[b]
\caption{Pixel-wise detection AUC obtained with the residual- and uncertainty-based detection methods\tnote{a}. }
\label{table:summary_pixel-wise}
%\centering
\scriptsize
%\resizebox{\textwidth}{!}{

\newcommand\len{0.68}

\begin{tabularx}{8.9cm}{@{}llp{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}@{}} \toprule


\multicolumn{2}{l}{Network} & \multicolumn{2}{c}{\textbf{AE}} & \multicolumn{3}{c}{\textbf{AESc}}  & \textbf{AE\textsubscript{L2}} & \textbf{AE\textsubscript{SSIM}} & \textbf{AnoGAN}\\

\arrayrulecolor{black!60}\cmidrule(lr){3-4}\cmidrule(lr){5-7}
\multicolumn{2}{l}{Corruption} & None & Stain & None & \multicolumn{2}{c}{Stain} & \cite{Bergmann2019} & \cite{Bergmann2019} & \cite{Bergmann2019}\\

\arrayrulecolor{black!60}\cmidrule(lr){6-7}
&&&&& Res. & Un. &&&\\

\arrayrulecolor{black!60}\midrule\midrule

 \multirow{5}{*}{\rotatebox[origin=c]{90}{Textures}} & Carpet & 0.57 & 0.62 & 0.52 & 0.79 & \textbf{0.91} & 0.59 & \underline{0.87} & 0.54\\
& Grid & 0.81 & 0.82 & 0.57 & 0.89 & \textbf{0.95} & 0.90  & \underline{0.94} & 0.58 \\
& Leather & 0.79 & 0.82 & 0.71 & \textbf{0.95} & \underline{0.87} & 0.75 & 0.78 & 0.64\\ 
& Tile & 0.45 & 0.54 & 0.62 & \underline{0.74}  & \textbf{0.79} & 0.51 & 0.59 & 0.50 \\
& Wood & 0.64 & 0.71 & 0.65 & \textbf{0.84} & \textbf{0.84} & 0.73  & 0.73 & 0.62\\
\arrayrulecolor{black!60}\cmidrule(lr){2-10}
& Mean\tnote{b} & 0.65 & 0.70 & 0.61 & \underline{0.84} & \textbf{0.87} & 0.70 & 0.78 & 0.58\\
\arrayrulecolor{black!60}\midrule

 \multirow{10}{*}{\rotatebox[origin=c]{90}{Objects}} & Bottle &  0.85 & \underline{0.88} & 0.47 & 0.84 & \underline{0.88} & 0.86 & \textbf{0.93} & 0.86 \\
& Cable & 0.62 & 0.83 & 0.72 & \underline{0.85} & 0.84 & \textbf{0.86} & 0.82 & 0.78 \\
& Capsule & 0.87 & 0.87 & 0.63 & 0.83 & \underline{0.93} & 0.88 & \textbf{0.94} & 0.84  \\
& Hazelnut & 0.92 & 0.93 & 0.79 & 0.88 & 0.89 & \underline{0.95} & \textbf{0.97} & 0.87\\
& Metal Nut &  0.82 & 0.84 & 0.52 & 0.57 & 0.62 & \underline{0.86} & \textbf{0.89} & 0.76\\
& Pill  & 0.81 & 0.81 & 0.64 & 0.74 & 0.85 & 0.85 & \textbf{0.91} & \underline{0.87}\\
& Screw & 0.93 & 0.93 & 0.72 & 0.86 & \underline{0.95} & \textbf{0.96} & \textbf{0.96} & 0.80  \\
& Toothbrush & 0.92 & \underline{0.93} & 0.73 & \textbf{0.93} & \textbf{0.93} & \textbf{0.93} & \underline{0.92} & 0.90\\
& Transistor & 0.79 & 0.82 & 0.56 & 0.80 & 0.78 & \underline{0.86} & \textbf{0.90} & 0.80 \\
& Zipper & 0.73 & 0.75 & 0.60 & 0.78 & \textbf{0.90} & 0.68 & \underline{0.88} & 0.78\\
\arrayrulecolor{black!60}\cmidrule(lr){2-10}
& Mean\tnote{c} & 0.83 & 0.86 & 0.64 & 0.81 & 0.86 & \underline{0.88} & \textbf{0.91} & 0.82\\
\arrayrulecolor{black!60}\midrule

& Global mean\tnote{d} & 0.77 & 0.81 & 0.63 & \underline{0.82} & \textbf{0.86} & 0.80 & \textbf{0.86} & 0.74 \\
\arrayrulecolor{black}\bottomrule

\end{tabularx}
\begin{tablenotes}
\item [a]For each row, the best performing approach is highlighted in boldface and the second best is underlined.
\item [b] Mean AUC obtained over the classes of images belonging to the texture categories.
\item [c] Mean AUC obtained over the classes of images belonging to the object categories.
\item [d] Mean AUC obtained over the entire dataset.
\end{tablenotes}
\end{threeparttable}

\vspace*{-0.2cm}
%}
\end{table}

==> Tables/SUMMARY_pixelandimage-wise.tex <==

\tabcolsep=0.03cm
\begin{table*}[!t]
\caption{Image- and pixel-wise detection AUC obtained with the residual- and uncertainty-based (only for pixel-wise) detection methods. For each row, the best performing approach for image- and pixel-wise detection, independently, is highlighted in boldface and the second best is underlined.}
\label{table:quantitativeRes}
\scriptsize
%\resizebox{\textwidth}{!}{

\newcommand\len{0.6}

\begin{tabularx}{11.3cm}{@{}l p{1.65 cm} p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{0.15 cm}p{\len cm}p{0.5 cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{0.1 cm}p{\len cm}p{\len cm}p{\len cm}p{\len cm}p{0.15 cm}p{1.05 cm}@{}} 
\arrayrulecolor{black}\cmidrule[0.8pt]{1-20}
&& \multicolumn{6}{c}{\textbf{Image-wise detection}} & & \multicolumn{11}{c}{\textbf{Pixel-wise detection}}  \\
\arrayrulecolor{black}\cmidrule[0.8pt]{3-8}\cmidrule[0.8pt]{10-20}


&& \multicolumn{6}{c}{\textbf{Residual}} & & \multicolumn{4}{c}{\textbf{Uncertainty}} && \multicolumn{6}{c}{\textbf{Residual}}  \\
\arrayrulecolor{black!60}\cmidrule(lr){3-8}\cmidrule(lr){10-13}\cmidrule(lr){14-20}
\multicolumn{2}{l}{Network} & \multicolumn{2}{c}{AE} & \multicolumn{2}{c}{AESc} && \multicolumn{2}{l}{ITAE \cite{Huang2019}} & \multicolumn{2}{c}{AE} & \multicolumn{2}{c}{AESc} && \multicolumn{2}{c}{AE} & \multicolumn{2}{c}{AESc} && AE\textsubscript{L2} \cite{Bergmann2019} \\
\arrayrulecolor{black!60}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){15-16}\cmidrule(lr){17-18}
\multicolumn{2}{l}{Corruption} & $~~~$- & Stain & $~~~$- & Stain &&&& $~~~$- & Stain & $~~~$- & Stain && $~~~$- & Stain & $~~~$- & Stain &&  \\

\arrayrulecolor{black!60}\cmidrule{1-20}
\arrayrulecolor{black!60}\cmidrule{1-20}

\multirow{6}{*}{\rotatebox[origin=c]{90}{Textures}} & Carpet & 0.43 & 0.43 & 0.48 & \textbf{0.89} && \underline{0.71} && 0.55 & 0.54 & 0.43 & \textbf{0.91} && 0.57 & 0.62 & 0.52 & \underline{0.79} && 0.59\\
& Grid & 0.80 & 0.84 & 0.52 & \textbf{0.97} && \underline{0.88} && 0.52 & 0.49 & 0.50 & \textbf{0.95} && 0.81 & 0.82 & 0.57 & 0.89 && \underline{0.90}\\
& Leather & 0.45 & 0.54 & 0.56 & \textbf{0.89} && \underline{0.87} &&  0.86 & 0.52 & 0.58 & \underline{0.87} && 0.79 & 0.82 & 0.71 & \textbf{0.95} && 0.75 \\
& Tile & 0.49 & 0.57 & \underline{0.88} & \textbf{0.99} && 0.74 && 0.54 & 0.50 & 0.53 & \textbf{0.79} && 0.45 & 0.54 & 0.62 & \underline{0.74} && 0.51\\
& Wood & 0.92 & \underline{0.94} & 0.92 & \textbf{0.95} && 0.92 && 0.61 & 0.48 & 0.51 & \textbf{0.84} && 0.64 & 0.71 & 0.65 & \textbf{0.84} && \underline{0.73}\\
\arrayrulecolor{black!60}\cmidrule{2-20}
& Mean & 0.62 & 0.66 & 0.67 & \textbf{0.94} && \underline{0.82} && 0.62 & 0.51 & 0.51 & \textbf{0.87} && 0.65 & 0.70 & 0.61 & \underline{0.84}  && 0.70\\
\arrayrulecolor{black!60}\cmidrule{1-20}

\multirow{11}{*}{\rotatebox[origin=c]{90}{Objects}} & Bottle & \textbf{0.98} & \underline{0.97} & 0.77 & \textbf{0.98} && 0.94 && 0.68 & 0.63 & 0.64 & \textbf{0.88} && 0.85 & \textbf{0.88} & 0.47 & 0.84 && \underline{0.86} \\
& Cable & 0.70 & 0.77 & 0.55 & \textbf{0.89} && \underline{0.83} && 0.54 & 0.70 & 0.66 & 0.84 && 0.62 & 0.83 & 0.72 & \underline{0.85} && \textbf{0.86}\\
& Capsule & \textbf{0.74} & 0.64 & 0.60 & \textbf{0.74} && \underline{0.68} && \underline{0.92} & 0.89 & 0.65 & \textbf{0.93} && 0.87 & 0.87 & 0.63 & 0.83  && 0.88 \\
& Hazelnut & \underline{0.90} & 0.88 & 0.85 & \textbf{0.94} && 0.86 && \textbf{0.95} & 0.91 & 0.60 & 0.89 && 0.92 & \underline{0.93} & 0.79 & 0.88 && \textbf{0.95} \\
& Metal Nut & 0.57 & 0.59 & 0.24 & \textbf{0.73} && \underline{0.67} && 0.79 & 0.73 & 0.50 & 0.62 &&  0.82 & \underline{0.84} & 0.52 & 0.57 && \textbf{0.86} \\
& Pill & 0.76 & 0.76 & 0.70 & \textbf{0.84} && \underline{0.79} && \underline{0.82} & \underline{0.82} & 0.61 & \textbf{0.85} && 0.81 & 0.81 & 0.64 & 0.74 && \textbf{0.85}\\
& Screw & 0.68 & 0.60 & 0.30 & \underline{0.74} && \textbf{1.00} && 0.94 & 0.94 & 0.61 & \underline{0.95} && 0.93 & 0.93 & 0.72 & 0.86 && \textbf{0.96} \\
& Toothbrush & 0.93 & \underline{0.96} & 0.78 & \textbf{1.00} && \textbf{1.00} && 0.84 & 0.83 & 0.79 & \textbf{0.93} && \underline{0.92} & \textbf{0.93} & 0.73 & \textbf{0.93} && \textbf{0.93}\\
& Transistor & 0.84 & \underline{0.85} & 0.46 & \textbf{0.91} && 0.84 && 0.79 & 0.64 & 0.51 & 0.78 && 0.79 & \underline{0.82} & 0.56 & 0.80 && \textbf{0.86}\\
& Zipper & \underline{0.90} & 0.88 & 0.72 & \textbf{0.94} && 0.80 && \underline{0.78} & 0.77 & 0.60 & \textbf{0.90} && 0.73 & 0.75 & 0.60 & \underline{0.78} && 0.77\\
\arrayrulecolor{black!60}\cmidrule{2-20}
& Mean  & 0.80 & 0.79 & 0.60 & \textbf{0.87} && \underline{0.84} && 0.81 & 0.79 & 0.62 & \underline{0.86} && 0.83 & \underline{0.86} & 0.64 & 0.81 && \textbf{0.88} \\
\arrayrulecolor{black!60}\cmidrule{1-20}
& Global mean & 0.74 & 0.75 & 0.62 & \textbf{0.89} && \underline{0.84} && 0.74 & 0.69 & 0.58 & \textbf{0.86} && 0.77 & 0.81 & 0.63 & \underline{0.82}  && \underline{0.82} \\
\arrayrulecolor{black}\cmidrule[0.8pt]{1-20}

\end{tabularx}
%}
\end{table*}



==> imgs/Architecture/tikz_architecture.tex <==
\tikzstyle{graysum} = [draw=myorange, fill=myorange!100, circle, node distance=0.2cm]

\begin{tikzpicture}
%\draw[use as bounding box, transparent] (-1.8,-1.8) rectangle (17.2, 3.2);
% Define the macro.
% 1st argument: Height and width of the layer rectangle slice.
% 2nd argument: Depth of the layer slice
% 3rd argument: X Offset --> use it to offset layers from previously drawn layers.
% 4th argument: Options for filldraw.
% 5th argument: Text to be placed below this layer.
% 6th argument: Y Offset --> Use it when an output needs to be fed to multiple layers that are on the same X offset.
\newcommand{\networkLayer}[7]{
\def\a{#1} % Used to distinguish input resolution for current layer.
\def\b{0.02}
\def\c{#2} % Width of the cube to distinguish number of input channels for current layer.
\def\t{#3} % X offset for current layer.
\def\d{#4} % Y offset for current layer.	
\coordinate (#7) at (\t+\c/2,\a/2,\d+\a/2);
% Draw the layer body.
\draw[line width=0.5mm](\c+\t,0,\d) -- (\c+\t,\a,\d) -- (\t,\a,\d);                                                      % back plane
\draw[line width=0.5mm](\t,0,\a+\d) -- (\c+\t,0,\a+\d) node[midway,below] {#6} -- (\c+\t,\a,\a+\d) -- (\t,\a,\a+\d) -- (\t,0,\a+\d); % front plane
\draw[line width=0.5mm](\c+\t,0,\d) -- (\c+\t,0,\a+\d);
\draw[line width=0.5mm](\c+\t,\a,\d) -- (\c+\t,\a,\a+\d);
\draw[line width=0.5mm](\t,\a,\d) -- (\t,\a,\a+\d);
% Recolor visible surfaces
\filldraw[#5] (\t+\b,\b,\a+\d) -- (\c+\t-\b,\b,\a+\d) -- (\c+\t-\b,\a-\b,\a+\d) -- (\t+\b,\a-\b,\a+\d) -- (\t+\b,\b,\a+\d); % front plane
\filldraw[#5] (\t+\b,\a,\a-\b+\d) -- (\c+\t-\b,\a,\a-\b+\d) -- (\c+\t-\b,\a,\b+\d) -- (\t+\b,\a,\b+\d);
% Colored slice.
\ifthenelse {\equal{#5} {}}
{} % Do not draw colored slice if #4 is blank.
{\filldraw[#5] (\c+\t,\b,\a-\b+\d) -- (\c+\t,\b,\b+\d) -- (\c+\t,\a-\b,\b+\d) -- (\c+\t,\a-\b,\a-\b+\d);} % Else, draw a colored slice.
}

		% INPUT
		%\node[] (input image) at (-3.75,0.5) {\includegraphics[height=30mm]{lenna.png}};
		\newcommand\x{1.3}
		%networkLayer{3.5}{0.03}{-2.0}{-2.0}{\includegraphics[width=3cm]{Images/introDiagram/clean.png}}{};
		%\networkLayer{3.5}{0.03}{-2.0}{-2.0}{color=black!0}{$256{\times}256$}{input}
		\node[canvas is zy plane at x = 0.2, transform shape,anchor=south] at (-2.0,0.1){\includegraphics[width=4cm,height=4.5cm]{imgs/introDiagram/clean.png}};
		
		% SKIP CONNECTIONS
		\newcommand\bending{20}
		\draw [->,color=black!60,line width=0.9mm] 
		(6.5,-2.5) edge [bend left=\bending] (10.2,-2.5)
		(4.5,-1.3) edge [bend left=\bending] (12.3,-1.3)
		(2.8,-0.1) edge [bend left=\bending] (13.9,-0.1)
		(1.3,1.2) edge [bend left=\bending] (15.7,1.2)
		(-0.4,2.2) to [bend left=\bending] (17.5,2.2);
		\node at (8.25,-2.1) [graysum] (diffsign) {+};
		\node at (8.25,-0.5) [graysum] (diffsign) {+};
		\node at (8.25,1.05) [graysum] (diffsign) {+};
		\node at (8.25,2.6) [graysum] (diffsign) {+};
		\node at (8.25,3.95) [graysum] (diffsign) {+};

		% ENCODER
		\draw[every loop,line width=2.3mm,>=latex,draw=myorange,fill=myorange]
		(-1.9,1.1) edge[] (-1.9+\x,1.1)
		(-0.5,0.15) edge[] (-0.5+\x,0.15)
		(1.1,-0.75) edge[] (1.1+\x,-0.75)
		(2.7,-1.7) edge[] (2.7+\x,-1.7)
		(4.6,-2.6) edge[] (4.6+\x,-2.6)
		(6.3,-3.5) to[] (6.3+\x,-3.5);
		
		\networkLayer{3.5}{0.05}{0.0}{0.0}{black!60,fill opacity=0.4}{$128{\times}128{\times}16$}{input}
		\networkLayer{3.0}{0.1}{2.4}{2.0}{black!60,fill opacity=0.4}{$64{\times}64 {\times}32$}{conv1}	
		\networkLayer{2.5}{0.2}{4.7}{4.0}{black!60,fill opacity=0.4}{$32{\times}32{\times}64$}{conv2}
		\networkLayer{2.0}{0.4}{6.9}{6.0}{black!60,fill opacity=0.4}{$16{\times}16{\times}128$}{conv3}   
		\networkLayer{1.5}{0.8}{9.1}{8.0}{black!60,fill opacity=0.4}{$8{\times}8{\times}256$}{conv4}   
		\networkLayer{1.0}{1.6}{11.4}{10.0}{black!60,fill opacity=0.4}{$4{\times}4 {\times}512$}{conv5} 


		% DECODER\\
		\node at (18.2,1.6) [] {\textbf{\textcolor{myturquoise}{\Large ${\circledast}({\uparrow}2)$}}};
		%\node at (9.5,-2.9) [] {\textbf{\textcolor{myturquoise}{\Large ${\uparrow}2$}}};
		\draw[every loop,line width=2.3mm,>=latex,draw=myturquoise,fill=myturquoise]
		(17.5,1.0) edge[] (17.5+\x,1.0)
		(15.8,0.15) edge[] (15.8+\x,0.15)
		(14.0,-0.75) edge[] (14.0+\x,-0.75)
		(12.4,-1.7) edge[] (12.4+\x,-1.7)
		(10.8,-2.6) edge[] (10.8+\x,-2.6)
		(8.9,-3.5) to[] (8.9+\x,-3.5);	

		\networkLayer{1.5}{0.8}{13.5}{8.0}{black!60,fill opacity=0.4}{$~8{\times}8{\times} 256$}{deconv4} 
		\networkLayer{2.0}{0.4}{14.7}{6.0}{black!60,fill opacity=0.4}{$~16{\times}16{\times}128$}{deconv3}  
		\networkLayer{2.5}{0.2}{15.8}{4.0}{black!60,fill opacity=0.4}{$~32{\times}32{\times}64$}{deconv2}
		\networkLayer{3.0}{0.1}{16.9}{2.0}{black!60,fill opacity=0.4}{$~64{\times}64{\times}32$}{deconv1}
		\networkLayer{3.5}{0.1}{18.1}{0.0}{black!60,fill opacity=0.4}{$~128{\times}128{\times}16$}{deconv0}
		%\networkLayer{4.0}{0.05}{19.35}{-2.0}{black!60,fill opacity=0.4}{$~256{\times}256{\times}16$}{out}
		\node[canvas is zy plane at x = 0.2, transform shape,anchor=south,fill opacity=0.95] at (19.35,-0.0){\includegraphics[width=4cm,height=4.5cm]{imgs/introDiagram/clean.png}};
	
		
	% LEGEND
	\newcommand\mysize{2.5}
	\newcommand\xpos{22.5}
	\newcommand\ypos{4.0}
	\draw[every loop,line width=2.3mm,>=latex,draw=myorange,fill=myorange]
		(\xpos,\ypos) to[] (\xpos+\x,\ypos);
		\node (orange) at (\xpos+1.8,\ypos) [fontscale=\mysize,anchor=west] {\begin{varwidth}{8cm} 
		Strided convolution (5x5)\\
		+ BN + LeakyReLU
		\end{varwidth}};
		
	\draw[every loop,line width=2.3mm,>=latex,draw=myturquoise,fill=myturquoise]
		(\xpos,\ypos-2.5) to[] (\xpos+\x,\ypos-2.5);
		\node (orange) at (\xpos+1.8,\ypos-2.5) [fontscale=\mysize,anchor=west] {\begin{varwidth}{8cm} 
		Upsampling (${\uparrow}2$) \\
		+ Convolution (5x5) \\
		+ BN + LeakyReLU
		\end{varwidth}};
	
	\node at (\xpos+0.6,\ypos-4.3) [] {\textbf{\textcolor{myturquoise}{\Large ${\circledast}({\uparrow}2)$}}};
	\draw[every loop,line width=2.3mm,>=latex,draw=myturquoise,fill=myturquoise]
		(\xpos,\ypos-5.0) to[] (\xpos+\x,\ypos-5.0);
	\node (orange) at (\xpos+1.8,\ypos-5.0) [fontscale=\mysize,anchor=west] {\begin{varwidth}{8cm} 
		Upsampling (${\uparrow}2$) \\
		+ Strided convolution (5x5) \\
		+ Sigmoid
		\end{varwidth}};
		
	\draw [->,color=black!60,line width=0.9mm] 
		(\xpos,\ypos-7) to [bend left=\bending] (\xpos+\x,\ypos-7);
	\node at (\xpos+0.635,\ypos-6.9) [graysum] (diffsign) {+};
	\node (blue) at (\xpos+1.8,\ypos-7) [fontscale=\mysize,anchor=west] {\begin{varwidth}{6cm} 
		Addition (only for AESc)
		\end{varwidth}};
		
\end{tikzpicture}

==> imgs/Results/corruptionComparison.tex <==
\begin{tikzpicture}[node distance=0.5cm,>=latex', every text node part/.style={align=center}]

	\newcommand\xidt{0.2}
	\newcommand\imsize{1.5}
	\newcommand\vertshift{0.8}
	\newcommand\mysize{0.4}
	\newcommand\yidt{-3.4}
	
	% INPUT
	\node at (-2*\xidt,\vertshift) [fontscale=\mysize, text width=1.5cm] {\includegraphics[width=\imsize cm]{\inputPATH}};
	\node at (-2*\xidt-1.0,\vertshift) [fontscale=\mysize,rotate=90] {Input};
	
	% MASK
	\ifMC
	    \node at (-2*\xidt,-2*\vertshift) [fontscale=\mysize, text width=1.5cm] {\includegraphics[width=\imsize cm]{\maskPATH}};
        \node at (-2*\xidt-1.0,-2*\vertshift) [fontscale=\mysize,rotate=90] {Mask};
    \else
        \node at (-2*\xidt,-\vertshift) [fontscale=\mysize, text width=1.5cm] {\includegraphics[width=\imsize cm]{\maskPATH}};
        \node at (-2*\xidt-1.0,-\vertshift) [fontscale=\mysize,rotate=90] {Mask};
    \fi


	% Labels 
	\node at (\imsize/2+0*\xidt,\vertshift) [fontscale=\mysize,rotate=90] {Prediction};
	\node at (\imsize/2+0*\xidt,-\vertshift) [fontscale=\mysize,rotate=90] {Residual};
	\ifMC
	    \node at (\imsize/2+0*\xidt,-3*\vertshift) [fontscale=\mysize,rotate=90] {Uncertainty};
	\fi
	
	% color bar
	\node at (11*\imsize+9*\xidt,-\vertshift-0.05) [fontscale=\mysize, text width=1.5cm] {\includegraphics[height=1.5cm]{\colorbarResidualPATH}};
	\ifMC
	    \node at (9*\imsize+8*\xidt,-3*\vertshift-0.05) [fontscale=\mysize, text width=1.5cm] {\includegraphics[height=1.5cm]{\colorbarUncertaintyPATH}};
	\fi
	
	% CLEAN CAESSC2
	\iflegend
	    \node at (\imsize+2*\xidt,\vertshift+1.0) [fontscale=\mysize] {Identity};
	\fi
	\node at (\imsize+2*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAESSCpredPATH}};
	\node at (\imsize+2*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAESSCresidualPATH}};
    \ifMC
	    \node at (\imsize+2*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAESSCuncertaintyPATH}};
	\fi
	
	% DROPS CAESSC2
	\iflegend
	    \node at (2*\imsize+3*\xidt,\vertshift+1.0) [fontscale=\mysize] {Drops};
	\fi
	\node at (2*\imsize+3*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\dropsCAESSCpredPATH}};
	\node at (2*\imsize+3*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\dropsCAESSCresidualPATH}};
	\ifMC
    	\node at (2*\imsize+3*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\dropsCAESSCuncertaintyPATH}};
    \fi

	

	
	% Gaussian noise
	\iflegend
    	\node at (4.5*\imsize+5.5*\xidt,\vertshift+1.5) [fontscale=\mysize] {Gaussian noise};
    	\draw [color=black!60,line width=0.2mm] 
    		(2.5*\imsize+4*\xidt,\vertshift+1.25) edge [] (6.5*\imsize+7*\xidt,\vertshift+1.25);
    \fi
	
	% GAUSSIAN 10 CAESSC2
	\iflegend
	    \node at (3*\imsize+4*\xidt,\vertshift+1.0) [fontscale=\mysize] {$\sigma=0.1$};
	\fi
	\node at (3*\imsize+4*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianTENCAESSCpredPATH}};
	\node at (3*\imsize+4*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianTENCAESSCresidualPATH}};
	\ifMC
	    \node at (3*\imsize+4*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianTENCAESSCuncertaintyPATH}};
	\fi
	
	% GAUSSIAN 20 CAESSC2
	\iflegend
	    \node at (4*\imsize+5*\xidt,\vertshift+1.0) [fontscale=\mysize] {$\sigma=0.2$};
	\fi
	\node at (4*\imsize+5*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianTWENTYCAESSCpredPATH}};
	\node at (4*\imsize+5*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianTWENTYCAESSCresidualPATH}};
	\ifMC
	    \node at (4*\imsize+5*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianTWENTYCAESSCuncertaintyPATH}};
	\fi
	
	% GAUSSIAN 40 CAESSC2
	\iflegend
	    \node at (5*\imsize+6*\xidt,\vertshift+1.0) [fontscale=\mysize] {$\sigma=0.4$};
	\fi
	\node at (5*\imsize+6*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianFORTYCAESSCpredPATH}};
	\node at (5*\imsize+6*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianFORTYCAESSCresidualPATH}};
	\ifMC
	    \node at (5*\imsize+6*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianFORTYCAESSCuncertaintyPATH}};
	\fi
	
	% GAUSSIAN 80 CAESSC2
	\iflegend
	    \node at (6*\imsize+7*\xidt,\vertshift+1.0) [fontscale=\mysize] {$\sigma=0.8$};
	\fi
	\node at (6*\imsize+7*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianEIGHTYCAESSCpredPATH}};
	\node at (6*\imsize+7*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianEIGHTYCAESSCresidualPATH}};
	\ifMC
	    \node at (6*\imsize+7*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\gaussianEIGHTYCAESSCuncertaintyPATH}};
	\fi
	
	
	% SCRATCH CAESSC2
	\iflegend
	    \node at (7*\imsize+8*\xidt,\vertshift+1.0) [fontscale=\mysize] {Scratch};
	\fi
	\node at (7*\imsize+8*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\scratchCAESSCpredPATH}};
	\node at (7*\imsize+8*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\scratchCAESSCresidualPATH}};
	\ifMC
	    \node at (7*\imsize+8*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\scratchCAESSCuncertaintyPATH}};
    \fi
    
    % STAIN CAESSC2
    \iflegend
	    \node at (8*\imsize+9*\xidt,\vertshift+1.0) [fontscale=\mysize] {Stain};
	\fi
	\node at (8*\imsize+9*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAESSCpredPATH}};
	\node at (8*\imsize+9*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAESSCresidualPATH}};
	\ifMC
	    \node at (8*\imsize+9*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAESSCuncertaintyPATH}};
    \fi
    
    
    % STAIN CAESSC2
    \iflegend
	    \node at (9*\imsize+10*\xidt,\vertshift+1.0) [fontscale=\mysize] {Mix1};
	\fi
	\node at (9*\imsize+10*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\structuralCAESSCpredPATH}};
	\node at (9*\imsize+10*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\structuralCAESSCresidualPATH}};
	\ifMC
	    \node at (9*\imsize+10*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\structuralCAESSCuncertaintyPATH}};
    \fi
    
        % STAIN CAESSC2
    \iflegend
	    \node at (10*\imsize+11*\xidt,\vertshift+1.0) [fontscale=\mysize] {Mix2};
	\fi
	\node at (10*\imsize+11*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainGaussianCAESSCpredPATH}};
	\node at (10*\imsize+11*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainGaussianCAESSCresidualPATH}};
	\ifMC
	    \node at (10*\imsize+11*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainGaussianCAESSCuncertaintyPATH}};
    \fi
	
	\end{tikzpicture}

==> imgs/Results/corruptionComparison_WoodReal6.tex <==
{ % handle local Path variables

\newif\ifMC
    %\MCtrue  % uncomment for a figure with MC outputs
    \MCfalse  % uncomment for a figure without MC outputs
    
\newif\iflegend
    %\legendtrue  % uncomment for a figure with legend
    \legendfalse  % uncomment for a figure without legend

\newcommand\inputPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_INPUT.png}
\newcommand\maskPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_GT.png}
\newcommand\colorbarResidualPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_COLORBAR.png}
\newcommand\colorbarUncertaintyPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6MC__COLORBAR.png}

\newcommand\CAESSCpredPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\CAESSCresidualPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\CAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}

\newcommand\stainCAESSCpredPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\stainCAESSCresidualPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\stainCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}

\newcommand\dropsCAESSCpredPATH{imgs/Prediction_analysis/Wood_VariedDrops256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\dropsCAESSCresidualPATH{imgs/Prediction_analysis/Wood_VariedDrops256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\dropsCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_VariedDrops256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}

\newcommand\scratchCAESSCpredPATH{imgs/Prediction_analysis/Wood_VariedScratch256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\scratchCAESSCresidualPATH{imgs/Prediction_analysis/Wood_VariedScratch256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\scratchCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_VariedScratch256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}


\newcommand\structuralCAESSCpredPATH{imgs/Prediction_analysis/Wood_Structural256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\structuralCAESSCresidualPATH{imgs/Prediction_analysis/Wood_Structural256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\structuralCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_Structural256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}

\newcommand\stainGaussianCAESSCpredPATH{imgs/Prediction_analysis/Wood_StainOrGaussian256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\stainGaussianCAESSCresidualPATH{imgs/Prediction_analysis/Wood_StainOrGaussian256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\stainGaussianCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_StainOrGaussian256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}


\newcommand\gaussianTENCAESSCpredPATH{imgs/Prediction_analysis/Wood_Gaussian10256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\gaussianTENCAESSCresidualPATH{imgs/Prediction_analysis/Wood_Gaussian10256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\gaussianTENCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_Gaussian10256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}

\newcommand\gaussianTWENTYCAESSCpredPATH{imgs/Prediction_analysis/Wood_Gaussian20256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\gaussianTWENTYCAESSCresidualPATH{imgs/Prediction_analysis/Wood_Gaussian20256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\gaussianTWENTYCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_Gaussian20256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}

\newcommand\gaussianFORTYCAESSCpredPATH{imgs/Prediction_analysis/Wood_Gaussian40256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\gaussianFORTYCAESSCresidualPATH{imgs/Prediction_analysis/Wood_Gaussian40256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\gaussianFORTYCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_Gaussian40256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}

\newcommand\gaussianEIGHTYCAESSCpredPATH{imgs/Prediction_analysis/Wood_Gaussian80256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_OUTPUT.png}
\newcommand\gaussianEIGHTYCAESSCresidualPATH{imgs/Prediction_analysis/Wood_Gaussian80256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_6_HEATMAP.png}
\newcommand\gaussianEIGHTYCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_Gaussian80256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_6_VARIANCEMC.png}

\includestandalone[width=12cm]{imgs/Results/corruptionComparison}

}


==> imgs/Results/smallComparison.tex <==
\begin{tikzpicture}[node distance=0.5cm,>=latex', every text node part/.style={align=center}]

	\newcommand\xidt{0.2}
	\newcommand\imsize{1.5}
	\newcommand\vertshift{0.8}
	\newcommand\mysize{0.4}
	\newcommand\yidt{-3.4}
	
	% INPUT
	\node at (-2*\xidt+0.3,\vertshift) [fontscale=\mysize, text width=1.5cm] {\includegraphics[width=\imsize cm]{\inputPATH}};
	\node at (-2*\xidt-1.0+0.3,\vertshift) [fontscale=\mysize,rotate=90] {Input};
	
	% MASK
	\ifMC
		\node at (-2*\xidt+0.3,-2*\vertshift) [fontscale=\mysize, text width=1.5cm] {\includegraphics[width=\imsize cm]{\maskPATH}};
    	\node at (-2*\xidt-1.0+0.3,-2*\vertshift) [fontscale=\mysize,rotate=90] {Mask};
	\else
        \node at (-2*\xidt+0.3,-\vertshift) [fontscale=\mysize, text width=1.5cm] {\includegraphics[width=\imsize cm]{\maskPATH}};
	    \node at (-2*\xidt-1.0+0.3,-\vertshift) [fontscale=\mysize,rotate=90] {Mask};
    \fi

	% Labels 
	\node at (\imsize/2+0*\xidt+0.15,\vertshift) [fontscale=\mysize,rotate=90] {Prediction};
	\node at (\imsize/2+0*\xidt+0.15,-\vertshift) [fontscale=\mysize,rotate=90] {Residual};
	\ifMC
	    \node at (\imsize/2+0*\xidt+0.15,-3*\vertshift) [fontscale=\mysize,rotate=90] {Uncertainty};
	\fi
	
	\iflegend
	    \node at (0.5*\imsize,\vertshift+1.4) [fontscale=\mysize,anchor=east] {Network};
	    \node at (0.5*\imsize,\vertshift+1.0) [fontscale=\mysize,anchor=east] {Corruption};
	\fi
	
	% color bar
	\node[anchor=east] at (5*\imsize+7.5*\xidt,-\vertshift-0.05) [fontscale=\mysize, text width=1.5cm] {\includegraphics[height=1.5cm]{\colorbarResidualPATH}};
	\ifMC
	    \node[anchor=east] at (5*\imsize+7.5*\xidt,-3*\vertshift-0.05) [fontscale=\mysize, text width=1.5cm] {\includegraphics[height=1.5cm]{\colorbarUncertaintyPATH}};
	\fi
	
	% CLEAN CAE2
	\iflegend
	    \node at (1.5*\imsize+2.5*\xidt,\vertshift+1.4) [fontscale=\mysize] {AE};
	    \draw [color=black!60,line width=0.2mm] 
    		(\imsize/2+2*\xidt+0.15,\vertshift+1.2) edge [] (5*\imsize/2+1*\xidt+0.15,\vertshift+1.2);
    	\node at (\imsize+2*\xidt,\vertshift+1.0) [fontscale=\mysize] {None};
    \fi
	\node at (\imsize+2*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAEpredPATH}};
	\node at (\imsize+2*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAEresidualPATH}};
	\ifMC
	    \node at (\imsize+2*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAEuncertaintyPATH}};
	\fi
	
	% STAIN CAE2
	\iflegend
	    \node at (2*\imsize+3*\xidt,\vertshift+1.0) [fontscale=\mysize] {Stain};
	\fi 
	\node at (2*\imsize+3*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAEpredPATH}};
	\node at (2*\imsize+3*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAEresidualPATH}};
	\ifMC
	    \node at (2*\imsize+3*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAEuncertaintyPATH}};
	\fi
	
	% CLEAN CAESSC2
	\iflegend
	    \node at (3.5*\imsize+4.5*\xidt,\vertshift+1.4) [fontscale=\mysize] {AESc};
	    \draw [color=black!60,line width=0.2mm] 
    		(5*\imsize/2+4*\xidt+0.15,\vertshift+1.2) edge [] (9*\imsize/2+3*\xidt+0.15,\vertshift+1.2);
	    \node at (3*\imsize+4*\xidt,\vertshift+1.0) [fontscale=\mysize] {None};
	\fi
	\node at (3*\imsize+4*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAESSCpredPATH}};
	\node at (3*\imsize+4*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAESSCresidualPATH}};
	\ifMC
	    \node at (3*\imsize+4*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\CAESSCuncertaintyPATH}};
	\fi
	
    % STAIN CAESSC2
    \iflegend
	    \node at (4*\imsize+5*\xidt,\vertshift+1.0) [fontscale=\mysize] {Stain};
	\fi
	\node at (4*\imsize+5*\xidt,\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAESSCpredPATH}};
	\node at (4*\imsize+5*\xidt,-\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAESSCresidualPATH}};
	\ifMC
	    \node at (4*\imsize+5*\xidt,-3*\vertshift) [fontscale=\mysize, text width=\imsize cm] {\includegraphics[width=1.5cm]{\stainCAESSCuncertaintyPATH}};
	\fi
	
	\end{tikzpicture}

==> imgs/Results/smallComparison_BottleReal13.tex <==
{ % handle local Path variables

\newif\ifMC
    %\MCtrue  % uncomment for a figure with MC outputs
    \MCfalse  % uncomment for a figure without MC outputs
    
\newif\iflegend
    %\legendtrue   % uncomment for a figure with legends
    \legendfalse % uncomment for a figure without legends
    
\newcommand\inputPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_INPUT.png}
\newcommand\maskPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_GT.png}
\newcommand\colorbarResidualPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_COLORBAR.png}
\newcommand\colorbarUncertaintyPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_13MC__COLORBAR.png}

\newcommand\CAEpredPATH{imgs/Prediction_analysis/Bottle_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_OUTPUT.png}
\newcommand\CAEresidualPATH{imgs/Prediction_analysis/Bottle_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_HEATMAP.png}
\newcommand\CAEuncertaintyPATH{imgs/Prediction_analysis/Bottle_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_13_VARIANCEMC.png}

\newcommand\stainCAEpredPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_OUTPUT.png}
\newcommand\stainCAEresidualPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_HEATMAP.png}
\newcommand\stainCAEuncertaintyPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_13_VARIANCEMC.png}

\newcommand\CAESSCpredPATH{imgs/Prediction_analysis/Bottle_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_OUTPUT.png}
\newcommand\CAESSCresidualPATH{imgs/Prediction_analysis/Bottle_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_HEATMAP.png}
\newcommand\CAESSCuncertaintyPATH{imgs/Prediction_analysis/Bottle_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_13_VARIANCEMC.png}

\newcommand\stainCAESSCpredPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_OUTPUT.png}
\newcommand\stainCAESSCresidualPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_13_HEATMAP.png}
\newcommand\stainCAESSCuncertaintyPATH{imgs/Prediction_analysis/Bottle_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_13_VARIANCEMC.png}


\includestandalone[width=7.5cm]{imgs/Results/smallComparison}

}


==> imgs/Results/smallComparison_CarpetReal20.tex <==
{ % handle local Path variables

\newif\ifMC
    \MCtrue  % uncomment for a figure with MC outputs
    %\MCfalse  % uncomment for a figure without MC outputs
    
\newif\iflegend
    \legendtrue   % uncomment for a figure with legends
    %\legendfalse % uncomment for a figure without legends
    
\newcommand\inputPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_INPUT.png}
\newcommand\maskPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_GT.png}
\newcommand\colorbarResidualPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_COLORBAR.png}
\newcommand\colorbarUncertaintyPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_20MC__COLORBAR.png}

\newcommand\CAEpredPATH{imgs/Prediction_analysis/Carpet_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_OUTPUT.png}
\newcommand\CAEresidualPATH{imgs/Prediction_analysis/Carpet_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_HEATMAP.png}
\newcommand\CAEuncertaintyPATH{imgs/Prediction_analysis/Carpet_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_20_VARIANCEMC.png}

\newcommand\stainCAEpredPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_OUTPUT.png}
\newcommand\stainCAEresidualPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_HEATMAP.png}
\newcommand\stainCAEuncertaintyPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_20_VARIANCEMC.png}

\newcommand\CAESSCpredPATH{imgs/Prediction_analysis/Carpet_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_OUTPUT.png}
\newcommand\CAESSCresidualPATH{imgs/Prediction_analysis/Carpet_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_HEATMAP.png}
\newcommand\CAESSCuncertaintyPATH{imgs/Prediction_analysis/Carpet_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_20_VARIANCEMC.png}

\newcommand\stainCAESSCpredPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_OUTPUT.png}
\newcommand\stainCAESSCresidualPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_20_HEATMAP.png}
\newcommand\stainCAESSCuncertaintyPATH{imgs/Prediction_analysis/Carpet_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_20_VARIANCEMC.png}


\includestandalone[width=6.1cm]{imgs/Results/smallComparison}

}


==> imgs/Results/smallComparison_WoodReal8.tex <==
{ % handle local Path variables

\newif\ifMC
    \MCtrue  % uncomment for a figure with MC outputs
    %\MCfalse  % uncomment for a figure without MC outputs
    
\newif\iflegend
    \legendtrue   % uncomment for a figure with legends
    %\legendfalse % uncomment for a figure without legends
    
\newcommand\inputPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_INPUT.png}
\newcommand\maskPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_GT.png}
\newcommand\colorbarResidualPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_COLORBAR.png}
\newcommand\colorbarUncertaintyPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_8MC__COLORBAR.png}

\newcommand\CAEpredPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_OUTPUT.png}
\newcommand\CAEresidualPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_HEATMAP.png}
\newcommand\CAEuncertaintyPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_8_VARIANCEMC.png}

\newcommand\stainCAEpredPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_OUTPUT.png}
\newcommand\stainCAEresidualPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_HEATMAP.png}
\newcommand\stainCAEuncertaintyPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAe2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_8_VARIANCEMC.png}

\newcommand\CAESSCpredPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_OUTPUT.png}
\newcommand\CAESSCresidualPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_HEATMAP.png}
\newcommand\CAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_Clean256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_8_VARIANCEMC.png}

\newcommand\stainCAESSCpredPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_OUTPUT.png}
\newcommand\stainCAESSCresidualPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/Real_8_HEATMAP.png}
\newcommand\stainCAESSCuncertaintyPATH{imgs/Prediction_analysis/Wood_VariedStain256x256_ImtoIm_CAeSSC2_d6_f5_n16_LR0.01RedOnPlateau_B16_Ep250_Gray_NoDA/MC_Real_8_VARIANCEMC.png}


\includestandalone[width=6.1cm]{imgs/Results/smallComparison}

}


==> imgs/introDiagram/tikzV1.tex <==

\tikzstyle{blueblock} = [draw=myblue, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.3mm]
\tikzstyle{boldblueblock} = [draw=myblue, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.85mm, opacity=0.4]
\tikzstyle{redblock} = [draw=mycrimson, rectangle, rounded corners, minimum height=3em, minimum width=6em]
\tikzstyle{boldredblock} = [draw=mycrimson, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.85mm, opacity=0.4]
\tikzstyle{anomalyblock} = [fill=mycrimson, rectangle, rounded corners, line width=0.7mm,opacity=0.2]
\tikzstyle{sum} = [draw=mycrimson, fill=white, circle]

\resizebox{0.8\textwidth}{!}{
\begin{tikzpicture}[node distance=2cm,>=latex', every text node part/.style={align=center}]

	\newcommand\mysize{0.4}
	\newcommand\tinysize{0.05}
	\newcommand\xx{-3.0}
	\newcommand\blocshift{3.0}   % Horizotal shift of corruption block
	\newcommand\blocshifty{1.4} % Vertical shift of corruption block 
	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TRAINING 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 %%%%%%% Training block %%%%%%%% 
\begin{scope}[yshift= 2 cm]
\node at (3.0,1.9) [boldblueblock, text width=14cm, text height=5.05cm] (training) {};
\node at (-2.1,4.3) [fontscale=\mysize] {\textcolor{myblue}{1. Phase d'entraînement}};
	
\node at (-3.0,1.65) [fontscale=\mysize, text width=1.5cm] (input) {\includegraphics[width=1.5cm]{imgs/introDiagram/clean.png}};

\node at (9.0,1.65) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/clean.png}};

\draw[->, line width=0.4mm, color = myblue, yshift=2.1cm]
	(-2.2,-0.5) edge [solid] (-1.3,-0.5)
	(4.35,-0.5) to [solid] (5.35,-0.5);

	%%%%%%% Corruption figures %%%%%%%% 
	\begin{scope}[xshift= 3 cm, yshift= 0 cm]
	\node at (-1.5,1.75) [blueblock,fontscale=\mysize, text width=5.3cm, text height=4.3cm] (corruption) {};
		
	\node at (-3.0,2.7) {\includegraphics[width=1.8cm]{imgs/introDiagram/stain.png}};
	\node at (-3.0,3.8) [fontscale=\mysize,color=myblue] {Stain}; 
	
	\node at (0.0,2.7) {\includegraphics[width=1.8cm]{imgs/introDiagram/scratch.png}};
	\node at (0.0,3.8) [fontscale=\mysize,color=myblue] {Scratch}; 
	
	\node at (-3.0,0.5) {\includegraphics[width=1.8cm]{imgs/introDiagram/drops.png}};
	\node at (-3.0,1.6) [fontscale=\mysize,color=myblue] {Drops}; 
	
	\node at (0.0,0.5) {\includegraphics[width=1.8cm]{imgs/introDiagram/gaussian.png}};
	\node at (0.0,1.6) [fontscale=\mysize,color=myblue] {Gaussian noise};
	
	\end{scope}
	


	%%%%%%% Network %%%%%%%% 
	\begin{scope}[xshift= 5.4 cm, yshift= -0.45 cm]
	
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (0,0.8) -- (0,-0.8) --(1.3,-0.4) -- (1.3,0.4) -- cycle; 
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (1.4,-0.4) -- (1.4,0.4) --(2.7,0.8) -- (2.7,-0.8) -- cycle;
	
	
	\draw[->,line width=0.2mm, color = orange,yshift=2.1cm]
	(0.3,0.72) edge [bend left=25,solid] (2.4,0.72)
	(0.65,0.6) edge [bend left=25,solid] (2.1, 0.6)
	(0.9,0.5) to [bend left=25,solid] (1.8, 0.5);

	\node at (0.2, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Encoder}; 
	\node at (2.55, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Decoder};
	\end{scope}
\end{scope}

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% INFERENCE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
\begin{scope}[yshift= -1.8 cm]

\node at (3.0,0.0) [boldredblock, text width=14cm, text height=5.5cm] (training) {};
\node at (-2.7,2.6) [fontscale=\mysize] {\textcolor{mycrimson}{2. Phase de test}};

\node at (-3.0,0) [fontscale=\mysize, text width=1.5cm] (input) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_INPUT.png}};

	%%%%%%% Network %%%%%%%% 
	\begin{scope}[xshift= -2.0 cm, yshift= -2.1cm]
	
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (0,0.8) -- (0,-0.8) --(1.3,-0.4) -- (1.3,0.4) -- cycle; 
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (1.4,-0.4) -- (1.4,0.4) --(2.7,0.8) -- (2.7,-0.8) -- cycle;
	
	\draw[->,line width=0.2mm, color = orange,yshift=2.1cm]
	(0.3,0.72) edge [bend left=25,solid] (2.4,0.72)
	(0.65,0.6) edge [bend left=25,solid] (2.1, 0.6)
	(0.9,0.5) to [bend left=25,solid] (1.8, 0.5);

	\node at (0.2, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Encoder}; 
	\node at (2.55, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Decoder};
	\end{scope}
	
% Residual-based detection
\begin{scope}[xshift= 0.2cm,yshift= 1.4cm]

\node at (1.7,0) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};

\node at (3.1,0) [sum,text width=0.2cm] (diff) {};
\node at (3.12,0) {\textcolor{mycrimson}{-}};

\node at (4.7,0.15) [anomalyblock,fontscale=\mysize, text width=1.55cm, text height=1.8cm] {};
\node at (4.7,0.15)[yshift=0.8cm]{\scriptsize \textcolor{mycrimson}{Anomaly map}};
\node at (4.7,0) [text width=1.5cm] (outvar) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_HEATMAP.png}};
\draw[->, line width=0.4mm, color = mycrimson]
	(-3.25,-0.65) -- (-3.25,0.95) --  (3.1,0.95) -- (3.1,0.2);
	\draw[->, line width=0.4mm, color = mycrimson]
	(2.45,0) edge (2.9,0)
	(3.4,0) to (3.8,0);

\draw[->, line width=0.4mm, color = mycrimson]
	(5.8,-0.1) edge [bend right=18,solid] (8.2,-0.6)
	(5.8,0.1) edge [bend left=30,solid] (6.3,0.6)
	(7.7,0.6) to [solid] (8.2,0.6);
\node at (9.0,-0.55) [text width=2.3cm,fontscale=\mysize] (det11) {\textcolor{mycrimson}{Pixel-wise detection}};
\node at (7.0,0.6) [text width=1.5cm, fontscale=\mysize] (l11) {\textcolor{mycrimson}{$L^2$ Norm}};
\node at (9.0,0.7) [text width=2.5cm, fontscale=\mysize] (det11) {\textcolor{mycrimson}{Image-wise detection}};
\end{scope}

\draw[line width=0.4mm, color = mycrimson, dashed] (1,0) -- (10.0,0);
	\node at (3,0.3) [fontscale=\mysize] (app1) {\textcolor{mycrimson}{\textit{Residual-based detection}}};
	\node at (3,-0.3) [fontscale=\mysize] (app1) {\textcolor{mycrimson}{\textit{Uncertainty-based detection}}};


% Uncertainty-based detection
\begin{scope}[xshift= 0.2cm, yshift= -1.7cm]

\node at (1.7+0.3,0.3) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7+0.2,0.2) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7+0.1,0.1) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7,0) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};

\node at (4.7,0.15) [anomalyblock,fontscale=\mysize, text width=1.55cm, text height=1.8cm] {};
\node at (4.7,0.15)[yshift=0.8cm]{\scriptsize \textcolor{mycrimson}{Anomaly map}};
\node at (4.7,0) [text width=1.5cm] (outvar) {\includegraphics[width=1.5cm]{imgs/introDiagram/MC_Real_90_VARIANCEMC.png}};

\draw[decorate,decoration={brace,amplitude=3pt,mirror}, line width=0.4mm, color = mycrimson] 
    (-2.1, 0.8) node(t_k_unten){} -- (0.4, 0.8) node(t_k_opt_unten){}; 
\node at (-0.8, -0.1) [fontscale=\mysize, text width=3.0cm] {\textcolor{mycrimson}{Monte Carlo dropout}};
\draw (-0.8, -0.05) [color= mycrimson,yshift=0.05cm] ellipse (1.05cm and 0.6cm);

\draw[->, line width=0.4mm, color = mycrimson]
	(0.4, 0.35+0.15) edge (0.8, 0.35+0.15)
	(0.4, 0.35-0.05) edge (0.8, 0.35-0.05)
	(0.4, 0.35-0.25) edge (0.8, 0.35-0.25)
	(0.4, 0.35-0.95) edge (0.8, 0.35-0.95)
	(2.9, 0.05) to (3.7, 0.05);
	\draw[line width=0.4mm, densely dotted,color = mycrimson]
	(0.55, -0.15) -- (0.55, -0.45);
	\node at (3.3, -0.2) [fontscale=\mysize, text width=3.0cm] {\textcolor{mycrimson}{$\sigma^2$}};


\draw[->, line width=0.4mm, color = mycrimson]
	(5.8,-0.1) edge [bend right=18,solid] (8.2,-0.6)
	(5.8,0.1) edge [bend left=30,solid] (6.3,0.6)
	(7.7,0.6) to [solid] (8.2,0.6);
\node at (9.0,-0.55) [text width=2.3cm,fontscale=\mysize] (det11) {\textcolor{mycrimson}{Pixel-wise detection}};
\node at (7.0,0.6) [text width=1.5cm, fontscale=\mysize] (l11) {\textcolor{mycrimson}{$L^2$ Norm}};
\node at (9.0,0.7) [text width=2.5cm, fontscale=\mysize] (det11) {\textcolor{mycrimson}{Image-wise detection}};
\end{scope}
	
\end{scope}

\end{tikzpicture}
}

==> imgs/introDiagram/tikz_introduction2.tex <==

\tikzstyle{blueblock} = [draw=bmvcblue, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.3mm]
\tikzstyle{boldblueblock} = [draw=bmvcblue, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.85mm, opacity=0.4]
\tikzstyle{redblock} = [draw=mycrimson, rectangle, rounded corners, minimum height=3em, minimum width=6em]
\tikzstyle{boldredblock} = [draw=mycrimson, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.85mm, opacity=0.4]
\tikzstyle{anomalyblock} = [fill=mycrimson, rectangle, rounded corners, line width=0.7mm,opacity=0.2]
\tikzstyle{sum} = [draw=mycrimson, fill=white, circle]

\begin{tikzpicture}[node distance=2cm,>=latex', every text node part/.style={align=center}]
	
	\newcommand\mysize{0.4}
	\newcommand\tinysize{0.05}
	\newcommand\xx{-3.0}
	\newcommand\blocshift{3.0}   % Horizotal shift of corruption block
	\newcommand\blocshifty{0.45} % Vertical shift of corruption block 
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% TRAINING 
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\node at (3.0,2.05+\blocshifty) [boldblueblock, text width=14cm, text height=6.8cm] (training) {};
	\node at (0.0,5.2+\blocshifty) [fontscale=\mysize] {\textcolor{bmvcblue}{1. Train on clean images with synthetic corruption}};
	
	\node at (\xx,1.65+\blocshifty) [fontscale=\mysize, text width=1.5cm] (input) {\includegraphics[width=1.5cm]{imgs/introDiagram/clean.png}};

	\node at (12.0+\xx,1.65+\blocshifty) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/clean.png}};

	% Corruption
	\node at (-1.5+\blocshift,1.75+\blocshifty) [blueblock,fontscale=\mysize, text width=5.3cm, text height=5.7cm] (corruption) {};
	
	\node at (-3.0+\blocshift,3.0+\blocshifty) [] (stain) {\includegraphics[width=2.2cm]{imgs/introDiagram/stain.png}};
	\node at (-3.0+\blocshift,4.4+\blocshifty) [fontscale=\mysize,color=bmvcblue] {Stain}; 
	
	\node at (0.0+\blocshift,3.0+\blocshifty) [] (scratch) {\includegraphics[width=2.2cm]{imgs/introDiagram/scratch.png}};
	\node at (0.0+\blocshift,4.4+\blocshifty) [fontscale=\mysize,color=bmvcblue] {Scratch}; 
	
	\node at (-3.0+\blocshift,-0.0+\blocshifty) [] (drops) {\includegraphics[width=2.2cm]{imgs/introDiagram/drops.png}};
	\node at (-3.0+\blocshift,1.4+\blocshifty) [fontscale=\mysize,color=bmvcblue] {Drops}; 
	
	\node at (0.0+\blocshift,-0.0+\blocshifty) [] (gaussian) {\includegraphics[width=2.2cm]{imgs/introDiagram/gaussian.png}};
	\node at (0.0+\blocshift,1.4+\blocshifty) [fontscale=\mysize,color=bmvcblue] {Gaussian noise}; 
	
	\newcommand\xa{8.3}      % horizontal shift of the network
	\newcommand\ya{0.8}      % network height (dim 2)
	\newcommand\shiftx{1.3}  % network width
	\newcommand\yb{0.4}      % network height (dim 1)
	
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (\xa+\xx,\ya) -- (\xa+\xx,-\ya) --(\xa+\shiftx+\xx,-\yb) -- (\xa+\shiftx+\xx,\yb) -- cycle; 
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (\xa+\shiftx+0.1+\xx,-\yb) -- (\xa+\shiftx+0.1+\xx,\yb) --(\xa+2*\shiftx+0.1+\xx,\ya) -- (\xa+2*\shiftx+0.1+\xx,-\ya) -- cycle;
	\draw[->,line width=0.2mm, color = orange,yshift=2.1cm]
	(1.05*\xa+1.05*\xx,0.9*\ya) edge [bend left=25,solid] (1.05*\xa+1.05*\xx+1.7*\shiftx,0.9*\ya)
	(1.1*\xa+1.1*\xx,0.8*\ya) edge [bend left=25,solid] (1.1*\xa+1.1*\xx+1.3*\shiftx,0.8*\ya)
	(1.15*\xa+1.15*\xx,0.7*\ya) to [bend left=25,solid] (1.15*\xa+1.15*\xx+0.9*\shiftx,0.7*\ya);

	
	\draw[->, line width=0.4mm, color = bmvcblue, yshift=2.1cm]
	(0.8+\xx,0.0) edge [solid] (1.6+\xx,0.0)
	(7.4+\xx,0.0) to [solid] (8.2+\xx,0.0);

	\node at (0.25+\xx+\xa,1.65+\blocshifty) [fontscale=\mysize,rotate=270,color=orange] {Encoder}; 
	\node at (-0.1+\xx+\xa+2*\shiftx,1.65+\blocshifty) [fontscale=\mysize,rotate=270,color=orange] {Decoder};
	%\node at (3.5,-1.6) [fontscale=\mysize,color=orange] {Mean Squared Error (MSE) minimisation};
	%\node at (6.0,5.0) [fontscale=\mysize,color=bmvcblue,align=right] {4 models of synthetic noise added during training};
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% INFERENCE
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\newcommand\xaa{-2.8}     % Horizontal shift of outputs
	\newcommand\yaa{-1.8}
	\newcommand\shiftxx{1.3}
	\newcommand\shifty{-4.8}  % vertical shift of the network
	\newcommand\ybb{1.5}      % Vertical shift between single output and MCDropout
	\newcommand\ymc{-0.4}      % Vertical shift of mcdropout output
	
	\node at (3.0,\shifty+0.3) [boldredblock, text width=14cm, text height=6.2cm] (training) {};
	\node at (0.5,3.1+\shifty) [fontscale=\mysize] {\textcolor{mycrimson}{2. Test on arbitrary images, i.e. with or without real defect}};
	
	% Input
	\node at (\xx,\shifty) [fontscale=\mysize, text width=1.5cm] (input) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_INPUT.png}};

	% Single output
	\node at (4.6+\xaa,\shifty+\ybb) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
	% Difference sign
	\node at (5.95+\xaa,\shifty+\ybb) [sum,text width=0.2cm] (diff) {};
	\node at (5.95+\xaa,\shifty+\ybb-0.04) {\textcolor{mycrimson}{-}};
	\draw[->, line width=0.4mm, color = mycrimson]
	(\xx,\shifty+0.75) -- (\xx,\shifty+2.65) --  (5.95+\xaa,\shifty+2.65) -- (5.95+\xaa,\shifty+\ybb+0.25);
	\draw[->, line width=0.4mm, color = mycrimson]
	(5.35+\xaa,\shifty+\ybb) edge (5.7+\xaa,\shifty+\ybb)
	(6.2+\xaa,\shifty+\ybb) to (6.55+\xaa,\shifty+\ybb);
	
	\node at (7.3+\xaa,\shifty+\ybb+0.15) [anomalyblock,fontscale=\mysize, text width=1.55cm, text height=1.8cm] {};
	\node at (7.3+\xaa,\shifty+\ybb+0.15)[yshift=0.8cm]{\footnotesize \textcolor{mycrimson}{Anomaly map}};
	
	\node at (7.3+\xaa,\shifty+\ybb) [text width=1.5cm] (outvar) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_HEATMAP.png}};

	
	\draw[->, line width=0.4mm, color = mycrimson]
	(8.3+\xaa,\shifty+\ybb-0.1) edge [bend right=18,solid] (11.0+\xaa,\shifty+\ybb-0.75)
	(8.3+\xaa,\shifty+\ybb+0.1) edge [bend left=30,solid] (8.8+\xaa,\shifty+\ybb+0.5)
	(10.3+\xaa,\shifty+\ybb+0.5) to [solid] (10.9+\xaa,\shifty+\ybb+0.5);
	
	\node at (11.9+\xaa,\shifty+\ybb-0.75) [text width=1.5cm,fontscale=\mysize] (det11) {\textcolor{mycrimson}{Pixel-wise detection}};
	\node at (9.5+\xaa,\shifty+\ybb+0.5) [text width=1.5cm, fontscale=\mysize] (l11) {\textcolor{mycrimson}{$L^2$ Norm}};
	\node at (11.9+\xaa,\shifty+\ybb+0.5) [text width=1.7cm, fontscale=\mysize] (det11) {\textcolor{mycrimson}{Image-wise detection}};
	
	
	% MCDropout output
	\node at (7.3+\xaa,\ymc+\shifty-\ybb+0.25) [anomalyblock,fontscale=\mysize, text width=1.55cm, text height=1.8cm] {};
	\node at (7.3+\xaa,\ymc+\shifty-\ybb+0.25)[yshift=-0.8cm]{\footnotesize \textcolor{mycrimson}{Anomaly map}};
	\node at (4.6+0.5+\xaa,\ymc+\shifty-\ybb+0.5) [text width=1.5cm] (mcout4) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
	\node at (7.3+\xaa,\ymc+\shifty-\ybb+0.4) [text width=1.5cm] (mcoutvar) {\includegraphics[width=1.5cm]{imgs/introDiagram/MC_Real_90_VARIANCEMC.png}};
	
	% ...
	%\draw[line width=0.4mm, densely dotted]
	%(4.6+1.0+\xaa,\shifty-\ybb-0.9) -- (4.6+1.2+\xaa,\shifty-\ybb-0.7);
	\node at (4.6+0.2+\xaa,\ymc+\shifty-\ybb+0.2) [text width=1.5cm] (mcout3) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
	\node at (4.6+0.1+\xaa,\ymc+\shifty-\ybb+0.1) [text width=1.5cm] (mcout2) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
	\node at (4.6+\xaa,\ymc+\shifty-\ybb) [text width=1.5cm] (mcout1) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
	
	% Ellipse with MC Dropout
	%\node at (mcout1.west) [fontscale=\mysize, text width=3.0cm, yshift=-0.3cm, xshift=-0.7cm, rotate=90] {\textcolor{mycrimson}{Monte Carlo Dropout}};
	%\draw (mcout1.west) [color= mycrimson,xshift=-0.85cm,yshift=-0.2cm] ellipse (0.6cm and 1.05cm);
	\node at (2.2+\xaa, \shifty-\ybb-0.5) [fontscale=\mysize, text width=3.0cm] {\textcolor{mycrimson}{Monte Carlo dropout}};
	\draw (2.2+\xaa, \shifty-\ybb-0.5) [color= mycrimson,yshift=0.05cm] ellipse (1.05cm and 0.6cm);
	\draw[->, line width=0.4mm, color = mycrimson]
	%(2.15+\xaa, \shifty-\ybb+0.8) edge (2.15+\xaa, \shifty-\ybb+0.15)
	(3.35+\xaa, \shifty-\ybb+0.15) edge (3.75+\xaa, \shifty-\ybb+0.15)
	(3.35+\xaa, \shifty-\ybb-0.05) edge (3.75+\xaa, \shifty-\ybb-0.05)
	(3.35+\xaa, \shifty-\ybb-0.25) edge (3.75+\xaa, \shifty-\ybb-0.25)
	(3.35+\xaa, \shifty-\ybb-0.95) edge (3.75+\xaa, \shifty-\ybb-0.95)
	(6.0+\xaa, \shifty-\ybb+0.05) to (6.45+\xaa, \shifty-\ybb+0.05);
	\draw[line width=0.4mm, densely dotted,color = mycrimson]
	(3.55+\xaa, \shifty-\ybb-0.45) -- (3.55+\xaa, \shifty-\ybb-0.75);
	\node at (6.2+\xaa, \shifty-\ybb-0.2) [fontscale=\mysize, text width=3.0cm] {\textcolor{mycrimson}{$\sigma^2$}};
	
	\draw[decorate,decoration={brace,amplitude=3pt,mirror}, line width=0.4mm, color = mycrimson] 
    (1.0+\xaa, \shifty-\ybb+0.55) node(t_k_unten){} -- 
    (3.3+\xaa, \shifty-\ybb+0.55) node(t_k_opt_unten){}; 
	
	%\draw[<->, line width=0.4mm, color = mycrimson]
	%(4.5+1.0+\xaa,\shifty-\ybb-1.3) -- (4.6+1.6+\xaa,\shifty-\ybb-0.6);
	%\node at (4.6+1.45+\xaa,\shifty-\ybb-0.95) [fontscale=\mysize,rotate=45,color=mycrimson, xshift=-0.2cm, yshift=-0.1cm] {Variance};
	
	\draw[->, line width=0.4mm, color = mycrimson]
	(8.3+\xaa,\shifty-\ybb-0.1) edge [bend right=18,solid] (11.0+\xaa,\shifty-\ybb-0.75)
	(8.3+\xaa,\shifty-\ybb+0.1) edge [bend left=30,solid] (8.8+\xaa,\shifty-\ybb+0.5)
	(10.3+\xaa,\shifty-\ybb+0.5) to [solid] (10.9+\xaa,\shifty-\ybb+0.5);
	
	\node at (11.9+\xaa,\shifty-\ybb-0.75) [text width=1.5cm,fontscale=\mysize] (det1) {\textcolor{mycrimson}{Pixel-wise detection}};
	\node at (9.5+\xaa,\shifty-\ybb+0.5) [text width=1.5cm, fontscale=\mysize] (l1) {\textcolor{mycrimson}{$L^2$ Norm}};
	\node at (11.9+\xaa,\shifty-\ybb+0.5) [text width=1.7cm, fontscale=\mysize] (det1) {\textcolor{mycrimson}{Image-wise detection}};
	
	% 2 methods 
	\draw[line width=0.4mm, color = mycrimson, dashed] (3.9+\xaa,\shifty) -- (12.75+\xaa,\shifty);
	\node at (5.8+\xaa,\shifty+0.35) [fontscale=\mysize] (app1) {\textcolor{mycrimson}{\textit{Residual-based detection}}};
	\node at (5.8+\xaa,\shifty-0.35) [fontscale=\mysize] (app1) {\textcolor{mycrimson}{\textit{Uncertainty-based detection}}};
	%\draw[line width=0.4mm, color = mycrimson, dashed] 
	%(3.9+\xaa,\shifty) -- (4.5+\xaa,\shifty)
	%(7.6+\xaa,\shifty) -- (12.75+\xaa,\shifty);
	%\node at (6.0+\xaa,\shifty) [fontscale=\mysize] (detection) {\textcolor{mycrimson}{2 detection methods}};
	
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,xshift=-7.3cm,yshift=-4.8cm] (\xa+\xx,\ya) -- (\xa+\xx,-\ya) --(\xa+\shiftx+\xx,-\yb) -- (\xa+\shiftx+\xx,\yb) -- cycle; 
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,xshift=-7.3cm,yshift=-4.8cm] (\xa+\shiftx+0.1+\xx,-\yb) -- (\xa+\shiftx+0.1+\xx,\yb) --(\xa+2*\shiftx+0.1+\xx,\ya) -- (\xa+2*\shiftx+0.1+\xx,-\ya) -- cycle;
	\draw[->,line width=0.2mm, color = orange,xshift=-7.3cm,yshift=-4.8cm]
	(1.05*\xa+1.05*\xx,0.9*\ya) edge [bend left=25,solid] (1.05*\xa+1.05*\xx+1.7*\shiftx,0.9*\ya)
	(1.1*\xa+1.1*\xx,0.8*\ya) edge [bend left=25,solid] (1.1*\xa+1.1*\xx+1.3*\shiftx,0.8*\ya)
	(1.15*\xa+1.15*\xx,0.7*\ya) to [bend left=25,solid] (1.15*\xa+1.15*\xx+0.9*\shiftx,0.7*\ya);
	
	\node at (1.25+\xx,\shifty) [fontscale=\mysize,rotate=270,color=orange] {Encoder};
	\node at (3.5+\xx,\shifty) [fontscale=\mysize,rotate=270,color=orange] {Decoder};
	
	%\draw[->, line width=0.4mm, color = orange]
	%(0.9+\xx,\shifty) to [solid] (2.0+\xx,\shifty);

\end{tikzpicture}

==> imgs/introDiagram/tikz_stainOnly.tex <==

\tikzstyle{blueblock} = [draw=myblue, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.3mm]
\tikzstyle{boldblueblock} = [draw=myblue, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.85mm, opacity=0.4]
\tikzstyle{redblock} = [draw=mycrimson, rectangle, rounded corners, minimum height=3em, minimum width=6em]
\tikzstyle{boldredblock} = [draw=mycrimson, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.85mm, opacity=0.4]
\tikzstyle{anomalyblock} = [fill=mycrimson, rectangle, rounded corners, line width=0.7mm,opacity=0.2]
\tikzstyle{sum} = [draw=mycrimson, fill=white, circle]

\resizebox{0.8\textwidth}{!}{
\begin{tikzpicture}[node distance=2cm,>=latex', every text node part/.style={align=center}]

	\newcommand\mysize{0.4}
	\newcommand\tinysize{0.05}
	\newcommand\xx{-3.0}
	\newcommand\blocshift{3.0}   % Horizotal shift of corruption block
	\newcommand\blocshifty{1.4} % Vertical shift of corruption block 
	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TRAINING 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 %%%%%%% Training block %%%%%%%% 
\begin{scope}[yshift= 1.8 cm]
\node at (3.0,2.15) [boldblueblock, text width=14cm, text height=3.05cm] (training) {};
\node at (2.8,3.5) [fontscale=\mysize] {\textcolor{myblue}{1. Train an autoencoder with skip connections on clean images corrupted with the Stain model}};
	
\node at (-1.9,1.65) [fontscale=\mysize, text width=1.5cm] (input) {\includegraphics[width=1.5cm]{imgs/introDiagram/clean.png}};

\node at (8.0,1.65) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/clean.png}};

	\draw[->, line width=0.4mm, color = myblue, yshift=2.1cm]
	(-0.9,-0.5) edge [solid] (0.1,-0.5)
	(3.0,-0.5) to [solid] (4.0,-0.5);

	%%%%%%% Corruption figures %%%%%%%% 
	\begin{scope}[xshift= 1.5 cm, yshift= 0.1 cm]
	\node at (0,1.68) [blueblock,fontscale=\mysize, text width=2.3cm, text height=1.90cm] (corruption) {};
	\node at (0,1.65) {\includegraphics[width=2.1cm]{imgs/introDiagram/stain.png}};
	\node at (0,3.0) [fontscale=\mysize,color=myblue] {Stain noise}; 
	\end{scope}
	
	%%%%%%% Network %%%%%%%% 
	\begin{scope}[xshift= 4.2 cm, yshift= -0.45 cm]
	
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (0,0.8) -- (0,-0.8) --(1.3,-0.4) -- (1.3,0.4) -- cycle; 
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (1.4,-0.4) -- (1.4,0.4) --(2.7,0.8) -- (2.7,-0.8) -- cycle;
	
	
	\draw[->,line width=0.2mm, color = orange,yshift=2.1cm]
	(0.3,0.72) edge [bend left=25,solid] (2.4,0.72)
	(0.65,0.6) edge [bend left=25,solid] (2.1, 0.6)
	(0.9,0.5) to [bend left=25,solid] (1.8, 0.5);

	\node at (0.2, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Encoder}; 
	\node at (2.55, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Decoder};
	\end{scope}
\end{scope}

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% INFERENCE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
\begin{scope}[yshift= -0.9 cm]

\node at (3.0,0.1) [boldredblock, text width=14cm, text height=5.6cm] (training) {};
\node at (0.2,2.7) [fontscale=\mysize] {\textcolor{mycrimson}{2. Test on arbitrary images, i.e. with or without real defect}};

\node at (-3.0,0) [fontscale=\mysize, text width=1.5cm] (input) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_INPUT.png}};

	%%%%%%% Network %%%%%%%% 
	\begin{scope}[xshift= -2.0 cm, yshift= -2.1cm]
	
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (0,0.8) -- (0,-0.8) --(1.3,-0.4) -- (1.3,0.4) -- cycle; 
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (1.4,-0.4) -- (1.4,0.4) --(2.7,0.8) -- (2.7,-0.8) -- cycle;
	
	\draw[->,line width=0.2mm, color = orange,yshift=2.1cm]
	(0.3,0.72) edge [bend left=25,solid] (2.4,0.72)
	(0.65,0.6) edge [bend left=25,solid] (2.1, 0.6)
	(0.9,0.5) to [bend left=25,solid] (1.8, 0.5);

	\node at (0.2, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Encoder}; 
	\node at (2.55, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Decoder};
	\end{scope}
	
% Residual-based detection
\begin{scope}[xshift= 0.2cm,yshift= 1.4cm]

\node at (1.7,0) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};

\node at (3.1,0) [sum,text width=0.2cm] (diff) {};
\node at (3.12,0) {\textcolor{mycrimson}{-}};

\node at (4.7,0.15) [anomalyblock,fontscale=\mysize, text width=1.55cm, text height=1.8cm] {};
\node at (4.7,0.15)[yshift=0.8cm]{\scriptsize \textcolor{mycrimson}{Anomaly map}};
\node at (4.7,0) [text width=1.5cm] (outvar) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_HEATMAP.png}};
\draw[->, line width=0.4mm, color = mycrimson]
	(-3.25,-0.65) -- (-3.25,0.95) --  (3.1,0.95) -- (3.1,0.2);
	\draw[->, line width=0.4mm, color = mycrimson]
	(2.45,0) edge (2.9,0)
	(3.4,0) to (3.8,0);

\draw[->, line width=0.4mm, color = mycrimson]
	(5.8,-0.1) edge [bend right=18,solid] (8.2,-0.6)
	(5.8,0.1) edge [bend left=30,solid] (6.3,0.6)
	(7.7,0.6) to [solid] (8.2,0.6);
\node at (9.0,-0.55) [text width=2.3cm,fontscale=\mysize] (det11) {\textcolor{mycrimson}{Pixel-wise detection}};
\node at (7.0,0.6) [text width=1.5cm, fontscale=\mysize] (l11) {\textcolor{mycrimson}{$L^2$ Norm}};
\node at (9.0,0.7) [text width=2.5cm, fontscale=\mysize] (det11) {\textcolor{mycrimson}{Image-wise detection}};
\end{scope}

\draw[line width=0.4mm, color = mycrimson, dashed] (1,0) -- (10.0,0);
	\node at (3,0.3) [fontscale=\mysize] (app1) {\textcolor{mycrimson}{\textit{Residual-based detection}}};
	\node at (3,-0.3) [fontscale=\mysize] (app1) {\textcolor{mycrimson}{\textit{Uncertainty-based detection}}};


% Uncertainty-based detection
\begin{scope}[xshift= 0.2cm, yshift= -1.7cm]

\node at (1.7+0.3,0.3) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7+0.2,0.2) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7+0.1,0.1) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7,0) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};

\node at (4.7,0.15) [anomalyblock,fontscale=\mysize, text width=1.55cm, text height=1.8cm] {};
\node at (4.7,0.15)[yshift=0.8cm]{\scriptsize \textcolor{mycrimson}{Anomaly map}};
\node at (4.7,0) [text width=1.5cm] (outvar) {\includegraphics[width=1.5cm]{imgs/introDiagram/MC_Real_90_VARIANCEMC.png}};

\draw[decorate,decoration={brace,amplitude=3pt,mirror}, line width=0.4mm, color = mycrimson] 
    (-2.1, 0.8) node(t_k_unten){} -- (0.4, 0.8) node(t_k_opt_unten){}; 
\node at (-0.8, -0.2) [fontscale=\mysize, text width=3.0cm] {\textcolor{mycrimson}{Monte Carlo dropout}};
\draw (-0.8, -0.15) [color= mycrimson,yshift=0.05cm] ellipse (1.05cm and 0.6cm);

\draw[->, line width=0.4mm, color = mycrimson]
	(0.4, 0.35+0.15) edge (0.8, 0.35+0.15)
	(0.4, 0.35-0.05) edge (0.8, 0.35-0.05)
	(0.4, 0.35-0.25) edge (0.8, 0.35-0.25)
	(0.4, 0.35-0.95) edge (0.8, 0.35-0.95)
	(2.9, 0.05) to (3.7, 0.05);
	\draw[line width=0.4mm, densely dotted,color = mycrimson]
	(0.55, -0.15) -- (0.55, -0.45);
	\node at (3.3, -0.2) [fontscale=\mysize, text width=3.0cm] {\textcolor{mycrimson}{$\sigma^2$}};


\draw[->, line width=0.4mm, color = mycrimson]
	(5.8,-0.1) edge [bend right=18,solid] (8.2,-0.6)
	(5.8,0.1) edge [bend left=30,solid] (6.3,0.6)
	(7.7,0.6) to [solid] (8.2,0.6);
\node at (9.0,-0.55) [text width=2.3cm,fontscale=\mysize] (det11) {\textcolor{mycrimson}{Pixel-wise detection}};
\node at (7.0,0.6) [text width=1.5cm, fontscale=\mysize] (l11) {\textcolor{mycrimson}{$L^2$ Norm}};
\node at (9.0,0.7) [text width=2.5cm, fontscale=\mysize] (det11) {\textcolor{mycrimson}{Image-wise detection}};
\end{scope}
	
\end{scope}

\end{tikzpicture}
}

==> imgs/introDiagram/tikz_stainOnly_large.tex <==

\tikzstyle{blueblock} = [draw=myblue, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.3mm]
\tikzstyle{boldblueblock} = [draw=myblue, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.85mm, opacity=0.4]
\tikzstyle{redblock} = [draw=mycrimson, rectangle, rounded corners, minimum height=3em, minimum width=6em]
\tikzstyle{boldredblock} = [draw=mycrimson, rectangle, rounded corners, minimum height=3em, minimum width=6em, line width=0.85mm, opacity=0.4]
\tikzstyle{anomalyblock} = [fill=mycrimson, rectangle, rounded corners, line width=0.7mm,opacity=0.2]
\tikzstyle{sum} = [draw=mycrimson, fill=white, circle]

%\resizebox{0.8\textwidth}{!}{
\begin{tikzpicture}[node distance=2cm,>=latex', every text node part/.style={align=center}]

	\newcommand\mysize{0.4}
	\newcommand\tinysize{0.05}
	\newcommand\xx{-3.0}
	\newcommand\blocshift{3.0}   % Horizotal shift of corruption block
	\newcommand\blocshifty{1.4} % Vertical shift of corruption block 
	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TRAINING 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 %%%%%%% Training block %%%%%%%% 
\begin{scope}[yshift= -2.5 cm]
\node at (2.5,2.4) [boldblueblock, text width=10.3cm, text height=4.3cm] (training) {};
\node at (-5.0,4.0) [fontscale=\mysize, text width=14cm, anchor=west] {\textcolor{myblue}{1. Train an autoencoder with skip connections on clean images}};
\node at (-6.85,3.6) [fontscale=\mysize, text width=14cm, anchor=west] {\textcolor{myblue}{corrupted with the Stain model}};

	
\node at (-1.8,1.65) [fontscale=\mysize, text width=1.5cm] (input) {\includegraphics[width=1.5cm]{imgs/introDiagram/clean.png}};

\node at (6.8,1.65) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/clean.png}};

	\draw[->, line width=0.4mm, color = myblue, yshift=2.1cm]
	(-1.0,-0.5) edge [solid] (-0.4,-0.5)
	(2.25,-0.5) to [solid] (2.9,-0.5);

	%%%%%%% Corruption figures %%%%%%%% 
	\begin{scope}[xshift= 1.0 cm, yshift= -0.1 cm]
	\node at (0,1.68) [blueblock,fontscale=\mysize, text width=2.3cm, text height=1.90cm] (corruption) {};
	\node at (0,1.65) {\includegraphics[width=2.1cm]{imgs/introDiagram/stain.png}};
	\node at (0,3.0) [fontscale=\mysize,color=myblue] {Stain noise}; 
	\end{scope}
	
	%%%%%%% Network %%%%%%%% 
	\begin{scope}[xshift= 3.0 cm, yshift= -0.45 cm]
	
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (0,0.8) -- (0,-0.8) --(1.3,-0.4) -- (1.3,0.4) -- cycle; 
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (1.4,-0.4) -- (1.4,0.4) --(2.7,0.8) -- (2.7,-0.8) -- cycle;
	
	
	\draw[->,line width=0.2mm, color = orange,yshift=2.1cm]
	(0.3,0.72) edge [bend left=25,solid] (2.4,0.72)
	(0.65,0.6) edge [bend left=25,solid] (2.1, 0.6)
	(0.9,0.5) to [bend left=25,solid] (1.8, 0.5);

	\node at (0.2, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Encoder}; 
	\node at (2.55, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Decoder};
	\end{scope}
\end{scope}

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% INFERENCE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
\begin{scope}[xshift=12.2cm, yshift= 0.0 cm]

\node at (3.0,0.2) [boldredblock, text width=14cm, text height=5.8cm] (training) {};
\node at (0.3,2.8) [fontscale=\mysize] {\textcolor{mycrimson}{2. Test on arbitrary images, i.e. with or without real defect}};

\node at (-3.0,0) [fontscale=\mysize, text width=1.5cm] (input) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_INPUT.png}};

	%%%%%%% Network %%%%%%%% 
	\begin{scope}[xshift= -2.0 cm, yshift= -2.1cm]
	
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (0,0.8) -- (0,-0.8) --(1.3,-0.4) -- (1.3,0.4) -- cycle; 
	\draw[fill=orange!60,fill opacity=0.4,draw=orange,yshift=2.1cm] (1.4,-0.4) -- (1.4,0.4) --(2.7,0.8) -- (2.7,-0.8) -- cycle;
	
	\draw[->,line width=0.2mm, color = orange,yshift=2.1cm]
	(0.3,0.72) edge [bend left=25,solid] (2.4,0.72)
	(0.65,0.6) edge [bend left=25,solid] (2.1, 0.6)
	(0.9,0.5) to [bend left=25,solid] (1.8, 0.5);

	\node at (0.2, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Encoder}; 
	\node at (2.55, 2.1) [fontscale=\mysize,rotate=270,color=orange] {Decoder};
	\end{scope}
	
% Residual-based detection
\begin{scope}[xshift= 0.2cm,yshift= 1.4cm]

\node at (1.7,0) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};

\node at (3.1,0) [sum,text width=0.2cm] (diff) {};
\node at (3.12,0) {\textcolor{mycrimson}{-}};

\node at (4.7,0.15) [anomalyblock,fontscale=\mysize, text width=1.55cm, text height=1.8cm] {};
\node at (4.7,0.15)[yshift=0.8cm]{\scriptsize \textcolor{mycrimson}{Anomaly map}};
\node at (4.7,0) [text width=1.5cm] (outvar) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_HEATMAP.png}};
\draw[->, line width=0.4mm, color = mycrimson]
	(-3.25,-0.65) -- (-3.25,0.95) --  (3.1,0.95) -- (3.1,0.2);
	\draw[->, line width=0.4mm, color = mycrimson]
	(2.45,0) edge (2.9,0)
	(3.4,0) to (3.8,0);

\draw[->, line width=0.4mm, color = mycrimson]
	(5.8,-0.1) edge [bend right=18,solid] (8.2,-0.6)
	(5.8,0.1) edge [bend left=30,solid] (6.3,0.6)
	(7.7,0.6) to [solid] (8.2,0.6);
\node at (9.0,-0.55) [text width=2.3cm,fontscale=\mysize] (det11) {\textcolor{mycrimson}{Pixel-wise detection}};
\node at (7.0,0.6) [text width=1.5cm, fontscale=\mysize] (l11) {\textcolor{mycrimson}{$L^2$ Norm}};
\node at (9.0,0.7) [text width=2.5cm, fontscale=\mysize] (det11) {\textcolor{mycrimson}{Image-wise detection}};
\end{scope}

\draw[line width=0.4mm, color = mycrimson, dashed] (1,0) -- (10.0,0);
	\node at (3,0.3) [fontscale=\mysize] (app1) {\textcolor{mycrimson}{\textit{Residual-based detection}}};
	\node at (3,-0.3) [fontscale=\mysize] (app1) {\textcolor{mycrimson}{\textit{Uncertainty-based detection}}};


% Uncertainty-based detection
\begin{scope}[xshift= 0.2cm, yshift= -1.7cm]

\node at (1.7+0.3,0.3) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7+0.2,0.2) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7+0.1,0.1) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};
\node at (1.7,0) [text width=1.5cm] (out) {\includegraphics[width=1.5cm]{imgs/introDiagram/Real_90_OUTPUT.png}};

\node at (4.7,0.15) [anomalyblock,fontscale=\mysize, text width=1.55cm, text height=1.8cm] {};
\node at (4.7,0.15)[yshift=0.8cm]{\scriptsize \textcolor{mycrimson}{Anomaly map}};
\node at (4.7,0) [text width=1.5cm] (outvar) {\includegraphics[width=1.5cm]{imgs/introDiagram/MC_Real_90_VARIANCEMC.png}};

\draw[decorate,decoration={brace,amplitude=3pt,mirror}, line width=0.4mm, color = mycrimson] 
    (-2.1, 0.8) node(t_k_unten){} -- (0.4, 0.8) node(t_k_opt_unten){}; 
\node at (-0.8, -0.2) [fontscale=\mysize, text width=3.0cm] {\textcolor{mycrimson}{Monte Carlo dropout}};
\draw (-0.8, -0.15) [color= mycrimson,yshift=0.05cm] ellipse (1.05cm and 0.6cm);

\draw[->, line width=0.4mm, color = mycrimson]
	(0.4, 0.35+0.15) edge (0.8, 0.35+0.15)
	(0.4, 0.35-0.05) edge (0.8, 0.35-0.05)
	(0.4, 0.35-0.25) edge (0.8, 0.35-0.25)
	(0.4, 0.35-0.95) edge (0.8, 0.35-0.95)
	(2.9, 0.05) to (3.7, 0.05);
	\draw[line width=0.4mm, densely dotted,color = mycrimson]
	(0.55, -0.15) -- (0.55, -0.45);
	\node at (3.3, -0.2) [fontscale=\mysize, text width=3.0cm] {\textcolor{mycrimson}{$\sigma^2$}};


\draw[->, line width=0.4mm, color = mycrimson]
	(5.8,-0.1) edge [bend right=18,solid] (8.2,-0.6)
	(5.8,0.1) edge [bend left=30,solid] (6.3,0.6)
	(7.7,0.6) to [solid] (8.2,0.6);
\node at (9.0,-0.55) [text width=2.3cm,fontscale=\mysize] (det11) {\textcolor{mycrimson}{Pixel-wise detection}};
\node at (7.0,0.6) [text width=1.5cm, fontscale=\mysize] (l11) {\textcolor{mycrimson}{$L^2$ Norm}};
\node at (9.0,0.7) [text width=2.5cm, fontscale=\mysize] (det11) {\textcolor{mycrimson}{Image-wise detection}};
\end{scope}
	
\end{scope}

\end{tikzpicture}
%}
